Influence Functions for Machine Learning: Nonparametric Estimators for Entropies, Divergences and Mutual Informations

We propose and analyze estimators for statistical functionals of one or more distributions under nonparametric assumptions. Our estimators are based on the theory of influence functions, which appear in the semiparametric statistics literature. We show that estimators based either on data-splitting or a leave-one-out technique enjoy fast rates of convergence and other favorable theoretical properties. We apply this framework to derive estimators for several popular information theoretic quantities, and via empirical evaluation, show the advantage of this approach over existing estimators.

==> appWorkedExample.tex <==

\section{Proofs of Results in Section~\ref{sec:workedExample}}
\label{sec:appWorkedExample}

\begin{proof}[Proof of Proposition~\ref{thm:tsalliscdInfFun}]
Recall that we can derive the influence functions via
$\psixz(X,Z_1; p) = \tsalliscd'_{XZ}(\delta_{X,Z_1}-\pxz; p)$, 
$\psiyz(Y,Z_2; p) = \tsalliscd'_{YZ}(\delta_{X,Z_2}-\pyz; p)$
% $\psixz(X,Z_1; \pxz, \pyz) = \tsalliscd'_{XZ}(\delta_{X,Z_1}-\pxz; \pxz,\pyz)$, 
% $\psiyz(Y,Z_2; \pxz, \pyz) = \tsalliscd'_{YZ}(\delta_{X,Z_2}-\pyz; \pxz,\pyz)$
where $\tsalliscd'_{XZ}, \tsalliscd'_{YZ}$ are the \gateaux derivatives of $\tsalliscd$
w.r.t $\pxz, \pyz$ respectively. Hence,
\begingroup
\allowdisplaybreaks
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  &\psixz(X,Z_1) = \\
  & \frac{1}{\alpha-1} \frac{\partial}{\partial t}
  \int ((1-t)\pxz + t\delta_{X Z_1})^\alpha \pyz^\beta \Big|_{t=0} \\
  & \frac{\alpha}{\alpha-1}\int\pxz^{\alpha-1} \pyz^\beta (\delta_{X Z_1} - \pxz) 
  \end{align*}
  }
  {
  \begin{align*}
  \psixz(X,Z_1) 
  &= \frac{1}{\alpha-1} \frac{\partial}{\partial t}
  \int ((1-t)\pxz + t\delta_{X Z_1})^\alpha \pyz^\beta \Big|_{t=0} \\
  &= \frac{\alpha}{\alpha-1}\int\pxz^{\alpha-1} \pyz^\beta (\delta_{X Z_1} - \pxz) 
  \end{align*}
  }
\endgroup
from which the result follows. Deriving $\psiyz$ is similar.
Alternatively, we can directly  show that $\psixz, \psiyz$ in Equation~\eqref{eqn:tsalliscdInfFun}
satisfy Definition~\ref{def:infFun}.
\end{proof}

To prove Corollary~\ref{thm:condTsallisAsympNormal} we will first need the
following Lemma. \\

\begin{lemma}
\label{lem:tsalliscdInfFunOrder}
Let $\phat = (\pxzhat, \pyzhat)$ be
a consistent estimator  for $p=(\pxz, \pyz)$. Then
$\EE_{XZ}\left[\left(\psixz(V; \phat) -   \psixz(V; p)\right)^2\right]$, 
$\EE_{YZ}\left[\left(\psiyz(W; \phat) -   \psiyz(W; p)\right)^2\right]$
$\in O(\|\pxz - \pxzhat\|^2 + \|\pyz - \pyzhat\|^2)$.
\begin{proof}
\vspace{-0.1in}
Given in Appendix~\ref{sec:appMultipleDistros}. It uses Jensen's
inequality and the boundedness of the densities.
\end{proof}
\begin{proof}
We will show this for $\EE_{XZ}\left[( \psixz(V;\phat) - \psixz(V;p) )^2
\right]$. The proof for $\EE_{YZ}\left[( \psiyz(W;\phat) - \psiyz(W;p) )^2
\right]$ is similar.
\begin{align*}
& \int \left( \psixz(u; \pxz, \pyz) - \psixz(u; \pxzhat, \pyzhat) \right)^2 \pxz\\
&\hspace{0.2in}= \frac{\alpha^2}{(1-\alpha)^2}
\int \left( \pxz^{\alpha-1}\pyz^\beta - \int \pxz^\alpha \pyz^\beta
  -\left[ \pxzhat^{\alpha-1}\pyzhat^\beta - \int \pxzhat^\alpha \pyzhat^\beta \right]
  \right)^2 \pxz \\
&\hspace{0.2in}\leq 2\frac{\alpha^2}{(1-\alpha)^2} \left[
\int \left(\pxz^{\alpha-1}\pyz^\beta - \pxzhat^{\alpha-1}\pyzhat^\beta \right)^2\pxz + 
\left( \int \pxz^\alpha \pyz^\beta - \int\pxzhat^\alpha \pyzhat^\beta \right)^2
\right] \\
&\hspace{0.2in}\leq 2\frac{\alpha^2}{(1-\alpha)^2} \left[
\int \left(\pxz^{\alpha-1}\pyz^\beta - \pxzhat^{\alpha-1}\pyzhat^\beta \right)^2\pxz + 
\int \left( \pxz^\alpha \pyz^\beta - \pxzhat^\alpha \pyzhat^\beta \right)^2
\right] \\
&\hspace{0.2in} \leq 4\frac{\alpha^2}{(1-\alpha)^2} \bigg[
\|\pyz^{\beta}\|_\infty^2 \int (\pxz^{\alpha-1} - \pxzhat^{\alpha-1})^2 +
\|\pxzhat^{\alpha-1}\|_\infty^2 \int (\pyz^\beta - \pyzhat^\beta)^2 + \\
&\hspace{0.6in}
\|\pyz^{\beta}\|_\infty^2 \int (\pxz^{\alpha} - \pxzhat^{\alpha})^2 +
\|\pxzhat^{\alpha}\|_\infty^2 \int (\pyz^\beta - \pyzhat^\beta)^2 
\bigg] \\
% &\hspace{0.2in}\in O\left(\|\pxz^{\alpha-1}\pyz^\beta -
% \pxzhat^{\alpha-1}\pyzhat^\beta\|^2 \right) +
% O\left( \|\pxz^\alpha \pyz^\beta - \pxzhat^\alpha \pyzhat^\beta\|^2 \right) \\
&\hspace{0.2in}\in
O\left( \|\pxz -\pxzhat\|^2 \right) +
O\left( \|\pyz -\pyzhat\|^2 \right) \rightarrow 0
\end{align*}
where, in the second and fourth steps we have used Jensen's inequality.
The last step follows from the boundedness of all our densities and estimates
and by lemma~\ref{lem:densitypowers}.
\end{proof}
\end{lemma}

We are now ready to prove asymptotic normality for the Conditional Tsallis
Estimator.

\begin{proof}[Proof of Corollary~\ref{thm:condTsallisAsympNormal}]
\vspace{-0.1in}
%% We need to verify that the following conditions hold. \begin{enumerate}
Recall that we need to verify the following: \begin{enumerate}
\item $\|\pxzhat - \pxz\|, \|\pyzhat - \pyz\| \in o_P(n^{-1/4})$
\item $\psixz(V; p), \psiyz(W; p)$ have bounded variance.
\item If $\|\pxzhat - \pxz\|, \|\pyzhat - \pyz\| \rightarrow 0$, then
  $\EE_{XZ} \left[\left(\psixz(V; \phat) -
  \psixz(V; p)\right)^2\right] \rightarrow 0$
  and  \\
  $\EE_{YZ}\left[\left(\psiyz(V; \phat) -
  \psiyz(W; p)\right)^2\right] \rightarrow 0$
\item $\psixz, \psiyz \neq \zero$.
\end{enumerate}
The first condition is true whenever $s > d/2$.
The second condition follows from the boundedness of the densities.
\begingroup
\allowdisplaybreaks
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  &\VV_{\pxz} \psixz(V;\pxz, \pyz) \\
  &\leq \frac{\alpha^2}{ (\alpha-1)^2 }
    \EE_{\pxz} \left[\pxz^{2\alpha-2}(X,Z_1) \pyz^{2\beta}(X,Z_1) \right] \\
  &= \frac{\alpha^2}{ (\alpha-1)^2 }\int \pxz^{2\alpha-1} \pyz^{2\beta} < \infty
  \end{align*}
  }
  {
  \begin{align*}
  \VV_{\pxz} \psixz(V;\pxz, \pyz) 
  &\leq \frac{\alpha^2}{ (\alpha-1)^2 }
    \EE_{\pxz} \left[\pxz^{2\alpha-2}(X,Z_1) \pyz^{2\beta}(X,Z_1) \right] \\
  &= \frac{\alpha^2}{ (\alpha-1)^2 }\int \pxz^{2\alpha-1} \pyz^{2\beta} < \infty
  \end{align*}
  }
\endgroup
We can bound $\VV_{\pyz}\psiyz$ similarly. The third condition follows from
Lemma~\ref{lem:tsalliscdInfFunOrder}.
For the fourth condition, note that when $\pxz = \pyz$,
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  &\psi_{XZ}(X,Z_1; \pxz, \pxz) \\
  &= \frac{\alpha}{\alpha -1} \left(
  \pxz^{\alpha+\beta-1}(X,Z_1) - \int \pxz\right) 
  = 0,
  \end{align*}
  }
  {
  \begin{align*}
  \psi_{XZ}(X,Z_1; \pxz, \pxz) 
  &= \frac{\alpha}{\alpha -1} \left(
  \pxz^{\alpha+\beta-1}(X,Z_1) - \int \pxz\right) 
  = 0,
  \end{align*}
  }
and similarly $\psi_{YZ} = \zero$.
Otherwise, $\psixz$ depends explicitly on $X,Z$ and is nonzero.
Therefore we have asymptotic normality away from $\pxz = \pyz$.
\end{proof}


==> expifml.tex <==

\vspace{-0.05in}
\section{Experiments}
\label{sec:experiments}
\vspace{-0.05in}

\insertFigToyOne
% \insertFigToyExamples

\subsection{Simulations}

First, we compare the estimators derived using our methods on a series of synthetic
examples in $1-4$ dimensions. 
% We compare against the methods in
% \cite{stowell2009fast,goria2005new,noughabi2013entropy,miller2003new,ramirez2009entropy,
% perez2008kullback,poczos12divergence,poczos2011estimation}. 
% Software for the
% estimators is obtained either directly from the papers or from~\citet{szabo14ite}.
For the \ds/\loos estimators, we estimate the density
via a KDE with the smoothing kernels constructed using
Legendre polynomials \citep{tsybakov08nonparametric}. 
In both cases and for 
the plug in estimator we choose the bandwidth by
performing $5$-fold cross validation. The integration for the plug in estimator
is approximated numerically.

We test the estimators on a series of synthetic datasets in $1-4$ dimension.
The specifics of the data generating distributions and methods compared to are given
below.
The results are shown in Figures~\ref{fig:toyOne} and~\ref{fig:toyTwo}. 
We make the
following observations. In most cases the \loos estimator performs best. The \dss
estimator approaches the \loos estimator when there are many samples but is generally 
inferior to the \loos estimator with few samples. This, as we have explained before is
because data splitting does not make efficient use of the data.
The \knns estimator for divergences
\cite{poczos12divergence} requires choosing a $k$. For this estimator,
 we used the default setting for $k$ given in the software.
As performance is sensitive to the choice of $k$, it performs well in some cases but
poorly in other cases.
We reiterate that our estimators do not require any setting of hyperparameters.

Next, we present some results on asymptotic normality. We test the \dss and
\loos estimators on a $4$-dimensional Hellinger divergence estimation problem. We use
$4000$ samples for estimation. We repeat this experiment $200$ times and compare the
empiritical asymptotic distribution (i.e. the $\sqrt{4000}(\widehat{T} -
T(f,g))/\widehat{S}$ values where $\widehat{S}$ is the estimated asymptotic
variance) to a $\Ncal(0,1)$ 
distribution on a QQ plot. The results in Figure~\ref{fig:toyTwo} suggest that both
estimators are asymptotically  normal. 
% We leave the question of resolving asymptotic
% normality of the \loos estimator to future work.

\textbf{Details: }
In our simulations, for the first figure comparing the Shannon Entropy
 in Fig~\ref{fig:toyOne} we generated data
from the following one dimensional density,
% \begin{equation*}
\[
f_1(t) = 0.5 + 0.5 t^9
\]
% \label{fig:toyExOne}
% \end{equation*}
For this, with probability $1/2$ we sample from the uniform distribution $U(0,1)$
on $(0,1)$ and otherwise sample $10$ points from $U(0,1)$ and pick the maximum.
For the third figure in Fig~\ref{fig:toyOne} comparing the KL divergence, we
generate data from the one dimensional density 
\[
f_2(t) = 0.5 + \frac{0.5t^{19}(1-t)^{19}}{B(20,20)}
\]
where $B(\cdot,\cdot)$ is the Beta function. For this, with probability $1/2$ we
sample from $U(0,1)$ and otherwise sample from a $\textrm{Beta}(20,20)$ distribution.
The second and fourth figures of Fig~\ref{fig:toyOne} we sampled from a $2$ dimensional
density where the first dimension was $f_1$ and the second was $U(0,1)$.
The fifth and sixth were from a $2$ dimensional
density where the first dimension was $f_2$ and the second was $U(0,1)$.
In all figures of Fig.~\ref{fig:toyTwo}, the first distribution was a $4$-dimensional density
where all dimensions are $f_2$. The latter was $U(0,1)^4$.

\textbf{Methods compared to: }
In addition to the plug-in, \dss and \loos estimators we perform comparisons with
several other estimators.
For the Shannon Entropy we compare our method to the \knns estimator of
\citet{goria2005new}, the method of \citet{stowell2009fast} which uses $K-D$
partitioning, the method of \citet{noughabi2013entropy} based on Vasicek's spacing
method and that of \citet{learned2003ica} based on Voronoi tessellation.
For the KL divergence we compare against the \knns method of \citet{perez2008kullback}
and that of \citet{ramirez2009entropy} based on the power spectral density
representation using Szego's theorem. For \renyi, \tsallis and Hellinger divergences
we compared against the \knns method of \citet{poczos12divergence}.
Software for these
estimators is obtained either directly from the papers or from~\citet{szabo14ite}.

\insertFigToyTwo

\subsection{Image Clustering Task}

Here we demonstrate a simple image clustering task using a nonparametric divergence
estimator. For this we use images from the ETH-80 dataset.
The objective here is not to champion our approach for image clustering against
all methods for image clustering out there. 
Rather, we just wish to demonstrate that our estimators can
be easily and intuitively applied to many Machine Learning problems.

We use the three categories Apples, Cows and Cups and randomly select $50$ images
from each category. Some sample images are shown in Fig~\ref{fig:clusImages}.
We convert the images to grey scale and extract the SIFT features from each
image. The SIFT features are $128$-dimensional but we project it to $4$ dimensions
via PCA. This is necessary because nonparametric methods work best in low dimensions.
Now we can treat each image as a collection of features, and hence a sample from a $4$
dimensional distribution. 
We estimate the Hellinger divergence between these ``distributions".
Then we construct an affinity matrix $A$ where the similarity metric between the
$i$\superscript{th} and $j$\superscript{th} image is given by $A_{ij} =
\exp(-\widehat{H}^2(X_i, X_j))$. Here $X_i$ and $X_j$ denotes the projected SIFT
samples from images $i$ and $j$ and $\widehat{H}(X_i, X_j)$ is the estimated
Hellinger divergence between the distributions.
Finally, we run a spectral clustering algorithm on the matrix $A$.


Figure~\ref{fig:affinity} depicts the affinity matrix $A$ when the images were
ordered according to their class label. The affinity matrix exhibits 
block-diagonal structure which indicates that our Hellinger divergence estimator
can in fact identify patterns in the images. 
Our approach achieved a clustering accuracy of $92.47\%$. When we used the $k$-NN
based estimator of~\cite{poczos12divergence} we achieved an accuracy of
$90.04\%$.
When we instead applied Spectral clustering naively, 
with $A_{ij} = \exp(-L_2(P_i,P_j)^2)$ where $L_2(P_i,P_j)$ is
the squared $L_2$ distance between the pixel intensities we achieved an accuracy of
$70.18\%$. We also tried $A_{ij} = \exp(-\alpha \widehat{H}^2(X_i, X_j))$ as the
affinity for
different choices of $\alpha$ and found that our estimator still performed best.
We also experimented with the
\renyi and \tsallis divergences and obtained similar results.

On the same note, one can imagine that these divergence estimators can also be used
for a classification task. For instance we can treat $\exp(-\widehat{H}^2(X_i, X_j))$
as a similarity
metric between the images and use it in a classifier such as an SVM.


\insertFigClustering


==> multipleDistros2.tex <==
\section{Functionals of Multiple Distributions}
\label{sec:multipleDistros}

\input{functionalEstimators}

We focus here on functionals of two distributions -- the extension to multiple
distributions is straightforward.
In the same vein to above, we will take $\Mcal$ to be the set of all measures
with densities in $L_2(\Xcal)$ and from now on write all derivatives in terms of
the functions.
The VME reduces to a Taylor expansion on the densities
(Lemma~\ref{lem:vmeTaylorEqTwoDistro}),
\begingroup
\allowdisplaybreaks
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  &T(q_1, q_2) 
     \numberthis \label{eqn:funcTaylorTwoDistro} \\
  &= T(p_1, p_2) + \phi'\left(\int \nu(p_1, p_2) \right)
    \int \partialfrac{p_1}{\nu} (q_1 - p_1) \\
    &\hspace{0.2in} + \phi'\left(\int \nu(p_1, p_2) \right)
    \int \partialfrac{p_2}{\nu} (q - p) + R_2   \\
    &= T(p_1, p_2) + \int \psi_1(\cdot; p_1, p_2) q_1 + 
     \int \psi_2(\cdot; p_1, p_2) q_2\\
    &\hspace{0.2in} + O \left( \|p_1 - q_1\|^2 +  \|p_2 - q_2\|^2 \right),
  \end{align*}
  }
  {
  \begin{align*}
  T(q_1, q_2) 
     \numberthis \label{eqn:funcTaylorTwoDistro} 
  &= T(p_1, p_2) + \phi'\left(\int \nu(p_1, p_2) \right)
    \int \partialfrac{p_1}{\nu} (q_1 - p_1) 
    + \phi'\left(\int \nu(p_1, p_2) \right)
    \int \partialfrac{p_2}{\nu} (q - p) + R_2   \\
  &= T(p_1, p_2) + \int \psi_1(\cdot; p_1, p_2) q_1 + 
     \int \psi_2(\cdot; p_1, p_2) q_2
    + O \left( \|p_1 - q_1\|^2 +  \|p_2 - q_2\|^2 \right),
  \end{align*}
  }
\endgroup
where $R_2 \in O \left( \|p_1 - q_1\|^2 +  \|p_2 - q_2\|^2 \right)$ if the second derivatives are bounded.
As before, we have replaced the first order terms with the corresponding terms in the VME.

The estimator for two distributions is analogous to the one distribution case.
Suppose we have samples $\Xonetwo\sim f$ and $\Yonetwo\sim g$.
 Let the influence functions of $T$ w.r.t
$f, g$ be $\psi_f, \psi_g$ respectively.
Use the first halves of the data $\Xone,
\Yone$ to construct density estimates $\fhat = \fhat(\Xone)$ and $\ghat = \ghat(\Yone)$. Then, use $\Xtwo, \Ytwo$ as follows: 
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  \Tf_1 &= T(\fhat, \ghat) +
    \frac{1}{n} \sum_{i=n+1}^{2n} \psi_f(X_i; \fhat, \ghat)  \\
  &\hspace{0.3in}
    + \frac{1}{m} \sum_{j=m+1}^{2m} \psi_g(Y_j; \fhat, \ghat) \numberthis
  \label{eqn:estimatorTwoDistro}
  \end{align*}
  }
  {
  \begin{align*}
  \Tf_1 &= T(\fhat, \ghat) +
    \frac{1}{n} \sum_{i=n+1}^{2n} \psi_f(X_i; \fhat, \ghat)  
%   &\hspace{0.3in}
    + \frac{1}{m} \sum_{j=m+1}^{2m} \psi_g(Y_j; \fhat, \ghat) \numberthis
  \label{eqn:estimatorTwoDistro}
  \end{align*}
  }
Finally, we swap the two samples $\Xone, \Xtwo$ to obtain $\Tf_2$ and then
compute $\Tf = (\Tf_1 + \Tf_2)/2$.

\subsection{Some Examples}
We demonstrate the applicability
of this framework by presenting estimators for some common functionals. %%  of one and two densities.
They are given in Table~\ref{tb:functionalDefns}.
% We provide a detailed derivation of the estimator and the analysis for the
% conditional Tsallis divergence in Section~\ref{sec:workedExample}.


While all estimators have been derived using our method of influence functions,
 we mention that for computational reasons this approach may not be desirable. 
For example, the estimator for \renyi divergence in Table~\ref{tb:functionalDefns} requires numerical integration.
This can be avoided by instead using an influence function-based estimator for $\int \px^\alpha \py^{1-\alpha}$ and passing this estimate through the $\log$ function. 

More generally, one can estimate a functional $\phi\left(\int \nu(p)\right)$ by first estimating $\int \nu(p)$ and plugging into $\phi$.
If $\int \nu(p)$ is bounded and $\phi$ is Lipschitz in that domain, then this
estimator achieves the same rates.
Furthery, by the Delta method they will also be asymptotically normal.
% , but it may \emph{not} be
% asymptotically normal.
% However, by the continuous mapping theorem, one can obtain asymptotic confidence intervals
% if $\phi$ is also continuous and one-to-one.
% \toworkon{Is this correct ? The Delta method would say that it is still
% asymptotically normal ??}

%% For the sake of consistency, we have used the influence functions of the
%% respective functionals  to obtain
%% the estimators. However, for computational considerations
%% we can derive alternative estimators using the same framework.
%% For instance, the estimator for the \renyi Divergence as
%% presented in the table require numerical integration. Alternatively we could
%% estimate $\int \px^\alpha \py^{1-\alpha}$ and plug that quantity back inside the
%% $\log$--via which we can avoid numeric integration.
%% More generally we can estimate the functional
%% $\phi\left(\int \nu(p)\right)$ by first estimating $\int \nu(p)$ and then
%% plugging it back. It can be shown that if $\int \nu(p)$ is bounded and $\phi$ is
%% Lipschitz in those bounds, that this estimator achieves the same rates.
%% This estimator will \emph{not} be asymptotically normal. But by the continuous
%% mapping theorem it is still
%% possible to obtain asymptotic confidence intervals if $\phi$ is also continuous
%% and one-to-one.



==> oneDistro2.tex <==

\section{Functionals of One Distribution}
\label{sec:oneDistro}

In this section, we focus on estimating a functional
$T(F) = T(f)= \phi(\int \nu(f) d\mu)$ (where $f$ is the density of $F$)
from samples $\Xonetwo \sim F$. 
Equation~\eqref{eqn:functaylor} leads to a natural estimator. 
If use half of the data $\Xone$ to construct a density estimator
$\fhat = \fhat(\Xone)$, then Equation~\eqref{eqn:functaylor} shows that:
\begin{align*}
T(f) - T(\fhat)  = \int \psi(x; \fhat)f(x)d\mu + O(\|f - \fhat\|_2^2)
\end{align*}
Since the influence function does not depend on the unknown distribution $F$,
the first term on the right hand side is simply an expectation.
We use the second half of the data to estimate this expectation with its sample mean.
This leads to the following preliminary estimator:
\begin{equation}
 \Tf_1 = T(\fhat) + \frac{1}{n}\sum_{i=n+1}^{2n} \psi(X_i; \fhat)
\label{eqn:estimator}
\end{equation}
We can similarly construct an estimator $\Tf_2$ by using $\Xtwo$ 
for density estimation and $\Xone$ for averaging. Our final estimator is
obtained via the average $\Tf =(\Tf_1+\Tf_2)/2$. While $\Tf_1$ itself attains
the correct rate of convergence using $\Tf$ will also give us the correct
constants in asymptotic normality.
% The estimator $\Tf_1$ has appeared in the literature
% and is typically analyzed for semiparametric 
% models~\cite{emery98probstat,robins09quadraticvm}.
% Building on this analysis we establish the following result for $\Tf$.
We establish the following result for $\Tf$. \\

\begin{theorem}[Bias, Variance, Asymptotic Normality]
Let $T$ have bounded second derivatives and $\psi$ be bounded. If $f \in
\Sigma(s,L)$
the Bias is $O\left(n^{\frac{-2s}{2s+d}}\right)$.
The Variance is
$O(n^{-1})$ when $s>d/2$ and $O\left(n^{\frac{-4s}{2s+d}}\right)$ otherwise.
Under certain regularity condtions, the estimator is asymptotically normal when
 $s > d/2$.
\end{theorem}

Even though our analysis of this estimator is new, we defer it to the appendix
since the result is incremental in comparison to \cite{robins09quadraticvm,
emery98probstat} who
analyse similar estimators in the Semiparametric setting.
However, we extend this analysis for functionals of multiple
distributions in the next section.



==> workedExample.tex <==
\section{An Illustrative Example}
\label{sec:workedExample}

Now, we present a step by step guide on applying our framework to
estimating any desired functional.
We choose the Conditional Tsallis divergence because pedagogically it is a
good example in Table~\ref{tb:functionalDefns} to illustrate the technique.
By following a similar procedure, one may derive an estimator for any desired
functional.

The Conditional \tsallis divergence
($\alpha \neq 0, 1$) between $X$ and $Y$ conditioned on $Z$  can be written
in terms of joint densities $\pxz, \pyz$. 
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  &\tsalliscd(p_{X|Z} \| p_{Y|Z}; p_Z) = \tsalliscd(\pxz, \pyz) =  \\
   &=\int  p_Z(z)\frac{1}{\alpha-1}\left(\int p_{X|Z}^{\alpha}(u,z)
      p_{Y|Z}^{1-\alpha}(u,z) \ud u -1\right) \ud z  \\
    &= \frac{1}{1- \alpha} + \frac{1}{\alpha-1}
    \int p^{\alpha}_{XZ}(u,z) p^{\beta}_{YZ}(u,z) \ud u \ud z
  \end{align*}
  }
  {
  \begin{align*}
  \tsalliscd(p_{X|Z} \| p_{Y|Z}; p_Z) = \tsalliscd(\pxz, \pyz) 
   &=\int  p_Z(z)\frac{1}{\alpha-1}\left(\int p_{X|Z}^{\alpha}(u,z)
      p_{Y|Z}^{1-\alpha}(u,z) \ud u -1\right) \ud z  \\
    &= \frac{1}{1- \alpha} + \frac{1}{\alpha-1}
    \int p^{\alpha}_{XZ}(u,z) p^{\beta}_{YZ}(u,z) \ud u \ud z
  \end{align*}
  }
where we have taken $\beta = 1-\alpha$. We have samples
% \footnote{Alternatively we
% could derive our estimators when samples are from the joint
% $(X_i, Y_i, Z_i)\sim\pxyz$, but we consider this setting because it is simpler.}
$V_i = (X_i, Z_{1i}) \sim \pxz, i = 1, \dots, 2n$
and $W_j = (Y_j,Z_{1j})\sim \pyz, j=1, \dots, 2m$
% and corresponds to the
% example provided in Section~\ref{sec:intro}.}.
We will assume $\pxz, \pyz \in \Sigma(s,L,B', B)$.
For brevity, we will write $p = (\pxz, \pyz)$ and $\phat = (\pxzhat, \pyzhat)$.

We begin with a functional Taylor expansion of $\tsalliscd(f,g)$ around
$(f_0, g_0)$. Since $\alpha, \beta \neq 0, 1$,
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  \tsalliscd(f,g) &=
    \tsalliscd(f_0, g_0) +
    \frac{\alpha}{\alpha - 1} \int f_0^{\alpha-1}g_0^\beta + \numberthis 
  \label{eqn:tsalliscdvme} \\
    & - \int f_0^{\alpha}g_0^{\beta-1} +
    O\left( \|f-f_0\|^2 + \|g-g_0\|^2 \right)
  \end{align*}
  }
  {
  \begin{align*}
  \tsalliscd(f,g) &=
    \tsalliscd(f_0, g_0) +
    \frac{\alpha}{\alpha - 1} \int f_0^{\alpha-1}g_0^\beta  \numberthis 
  \label{eqn:tsalliscdvme} 
     - \int f_0^{\alpha}g_0^{\beta-1} +
    O\left( \|f-f_0\|^2 + \|g-g_0\|^2 \right)
  \end{align*}
  }
We can bound the second order terms by  $O\left( \|f-f_0\|^2 + \|g-g_0\|^2
\right)$. Precisely, the second order
remainder is,
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
    &\frac{\alpha^2}{\alpha - 1} \int f_*^{\alpha-2}g_*^\beta (f - f_0)^2
    -\beta \int f_*^{\alpha}g_*^{\beta-2} (g - g_0)^2 \\
    &+\frac{\alpha\beta}{\alpha -1} \int f_*^{\alpha-1}g_*^{\beta} (f-f_0)(g-g_0) 
  \end{align*}
  }
  {
  \begin{align*}
    &\frac{\alpha^2}{\alpha - 1} \int f_*^{\alpha-2}g_*^\beta (f - f_0)^2
    -\beta \int f_*^{\alpha}g_*^{\beta-2} (g - g_0)^2 
    +\frac{\alpha\beta}{\alpha -1} \int f_*^{\alpha-1}g_*^{\beta} (f-f_0)(g-g_0) 
  \end{align*}
  }
where $(f_*,g_*)$ is in the line segment between $(f,g)$ and $(f_0,g_0)$.
If $f,g,f_0,g_0$ are bounded above and below so are $f_*, g_*$ and
 $ f_*^a g_*^b $ where $a,b$ are coefficients depending on $\alpha$.
The first two terms are respectively 
$O\left( \|f-f_0\|^2\right)$, $O\left(\|g-g_0\|^2 \right)$.
The cross term can be bounded via,
$\abr{\int (f-f_0)(g-g_0) } \leq \int \max\{ |f-f_0|^2, |g-g_0|^2 \} \in 
O( \|f-f_0\|^2 + \|g-g_0\|^2)$. We now state the influence functions of
$\tsalliscd$. The derivation is fairly straightforward using the \gateaux
derivative and is given in Appendix~\ref{sec:appWorkedExample}.
\\[\thmparaspacing]

\begin{proposition}[Influence Functions of $\tsalliscd$]
The influence functions of $\tsalliscd$ w.r.t $\pxz$, $\pyz$ are
\begingroup
\allowdisplaybreaks
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  &\psixz(X, Z_1; \pxz, \pyz) = \numberthis \label{eqn:tsalliscdInfFun} \\
  &\frac{\alpha}{\alpha-1}  \left(
    \pxz^{\alpha-1}(X,Z_1)\pyz^{\beta}(X,Z_1) - \int \pxz^\alpha\pyz^\beta  \right) \\
  &\psiyz(Y, Z_2; \pxz, \pyz) = \\
  & - \left(
  \pxz^{\alpha}(Y,Z_2)\pyz^{\beta-1}(Y,Z_2) - \int \pxz^\alpha\pyz^\beta  \right)
  \end{align*}
  }
  {
  \begin{align*}
  \psixz(X, Z_1; \pxz, \pyz) &= \numberthis \label{eqn:tsalliscdInfFun} 
  \frac{\alpha}{\alpha-1}  \left(
    \pxz^{\alpha-1}(X,Z_1)\pyz^{\beta}(X,Z_1) - \int \pxz^\alpha\pyz^\beta  \right) \\
  \psiyz(Y, Z_2; \pxz, \pyz) &= 
   - \left(
  \pxz^{\alpha}(Y,Z_2)\pyz^{\beta-1}(Y,Z_2) - \int \pxz^\alpha\pyz^\beta  \right)
  \end{align*}
  }
\endgroup
\label{thm:tsalliscdInfFun}
\end{proposition}
We use
$\Vone, \Wone$ to construct density estimates $\pxzhat, \pyzhat$ for $\pxz,
\pyz$. Then, use $\Vtwo, \Wtwo$ to add the sample means of the influence
functions given in
Theorem~\ref{thm:tsalliscdInfFun}. This results in our preliminary estimator, 
\begingroup
\allowdisplaybreaks
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  \tsalliscdestimss{1} &= \frac{1}{1 - \alpha} + \frac{\alpha}{\alpha-1}
    \frac{1}{n}\sum_{i=n+1}^{2n}
    \left( \frac{\pxzhat(X_i, Z_{1i})}{\pyzhat(X_i, Z_{1i})} \right)^{\alpha-1} \\
  &\hspace{0.2in}  - \frac{1}{m}\sum_{j=m+1}^{2m}
    \left( \frac{\pxzhat(Y_j, Z_{2j})}{\pyzhat(Y_j, Z_{2j})} \right)^{\alpha}
    \numberthis.
  \label{eqn:tsalliscdestim}
  \end{align*}
  }
  {
  \begin{align*}
  \tsalliscdestimss{1} &= \frac{1}{1 - \alpha} + \frac{\alpha}{\alpha-1}
    \frac{1}{n}\sum_{i=n+1}^{2n}
    \left(\frac{\pxzhat(X_i, Z_{1i})}{\pyzhat(X_i, Z_{1i})} \right)^{\alpha-1} 
    - \frac{1}{m}\sum_{j=m+1}^{2m}
    \left(\frac{\pxzhat(Y_j, Z_{2j})}{\pyzhat(Y_j, Z_{2j})} \right)^{\alpha}
    \numberthis.
  \label{eqn:tsalliscdestim}
  \end{align*}
  }
\endgroup
The final estimate is 
$\tsalliscdestim = (\tsalliscdestimss{1} + \tsalliscdestimss{2})/2$
where $\tsalliscdestimss{2}$ is obtained by swapping the two samples.
% When $\pxy,\pxz \in \Sigma(s, L)$, this estimator achieves 
% $O(n^{-1} + n^{\frac{-4s}{2s+d}})$ rate.
As mentioned earlier, the boundedness of the densities give us the rates in
Corollary~\ref{thm:ratesholder}.
To show asymptotic normality, we need to verify the conditions in
Theorem~\ref{thm:asympNormalTwoDistro}.
% \begin{enumerate}
% \item $\|\pxzhat - \pxz\|, \|\pyzhat - \pyz\| \in o_P(n^{-1/4})$
% \item $\psixz(V; p), \psiyz(W; p)$ have bounded variance.
% \item If $\|\pxzhat - \pxz\|, \|\pyzhat - \pyz\| \rightarrow 0$, then
%   $\EE_{XZ} \left[\left(\psixz(V; \phat) -
%   \psixz(V; p)\right)^2\right] \rightarrow 0$
%   and  \\
%   $\EE_{YZ}\left[\left(\psiyz(V; \phat) -
%   \psiyz(W; p)\right)^2\right] \rightarrow 0$
% \item $\psixz, \psiyz \neq \zero$.
% \end{enumerate}
This is a fairly routine excercise and we outline the steps in
Appendix~\ref{sec:appWorkedExample}.
We state the result formally below. \\

\begin{corollary}
\label{thm:tsalliscdAsympNormal}
Let $\pxy,\pxz \in \Sigma(s, L, B, B')$. Then $\tsalliscdestim$
% the estimator~\eqref{eqn:tsalliscdestim}
 is asymptotically normal when $\pxz \neq \pyz$ and  $s>d/2$.
\label{thm:condTsallisAsympNormal}
\end{corollary}

Finally, to construct a confidence interval we need a consistent
estimate of the asymptotic variance : 
$\frac{1}{\zeta} \VV_{XZ}\left[ \psixz(V; p) \right]
+ \frac{1}{1-\zeta} \VV_{YZ} \left[ \psiyz(W; p) \right]$ where,
\begingroup
\allowdisplaybreaks
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  & \VV_{XZ}\left[ \psixz(X, Z_1; \pxz, \pyz) \right] = \\ %%\numberthis 
  %%  \label{eqn:tsalliscdAsympVar}\\
  & \left( \frac{\alpha}{\alpha-1} \right)^2 \left( \int \pxz^{2\alpha-1}
  \pyz^{2\beta} - \left( \int \pxz^\alpha \pyz^\beta \right)^2 \right) \\
  & \VV_{YZ}\left[ \psiyz(Y, Z_2; \pxz, \pyz) \right] =  \\
  & \left( \int \pxz^{2\alpha}
  \pyz^{2\beta-1} - \left( \int \pxz^\alpha \pyz^\beta \right)^2 \right)
  \end{align*}
  }
  {
  \begin{align*}
   \VV_{XZ}\left[ \psixz(X, Z_1; \pxz, \pyz) \right] &=
  %%  \label{eqn:tsalliscdAsympVar}\\
  \left( \frac{\alpha}{\alpha-1} \right)^2 \left( \int \pxz^{2\alpha-1}
  \pyz^{2\beta} - \left( \int \pxz^\alpha \pyz^\beta \right)^2 \right) \\
  \VV_{YZ}\left[ \psiyz(Y, Z_2; \pxz, \pyz) \right] &=  
  \left( \int \pxz^{2\alpha}
  \pyz^{2\beta-1} - \left( \int \pxz^\alpha \pyz^\beta \right)^2 \right)
  \end{align*}
  }
\endgroup
From our analysis above, % of the \tsallis Conditional Divergence, we know that any
we know that any 
functional of the form $S(a,b) = \int \pxz^a \pyz^b$, $a+b=1, a,b\neq 0,1$
can be estimated via
\begin{align*}
\widehat{S}(a,b) =
\frac{a}{n}\sum_{i=n+1}^{2n}  \frac{\widehat{p}^b_{YZ}(V_i)}{\widehat{p}^b_{XZ}(V_i)} 
   + 
\frac{b}{m}\sum_{j=m+1}^{2m}  \frac{\widehat{p}^a_{XZ}(W_j)}{\widehat{p}^a_{YZ}(W_j)} 
\end{align*}
where $\pxzhat,\pyzhat$ are the density estimates from $\Vone, \Wone$.
$n/N$ is a consistent estimator for $\zeta$.
 This gives the following estimator for the asymptotic variance,
\ifthenelse{\boolean{istwocolumn}}
  {
  \begin{align*}
  &\frac{N}{n}\frac{\alpha^2}{(\alpha-1)^2} \widehat{S}(2\alpha-1, 2\beta)  +
  \frac{N}{m} \widehat{S}(2\alpha, 2\beta-1) \\
  &- 
   \frac{N (m\alpha^2 + n(\alpha-1)^2)}{nm(\alpha-1)^2}\widehat{S}^2(\alpha, \beta).
  \end{align*}
  }
  {
  \begin{align*}
  \frac{N}{n}\frac{\alpha^2}{(\alpha-1)^2} \widehat{S}(2\alpha-1, 2\beta)  +
  \frac{N}{m} \widehat{S}(2\alpha, 2\beta-1) - 
   \frac{N (m\alpha^2 + n(\alpha-1)^2)}{nm(\alpha-1)^2}\widehat{S}^2(\alpha, \beta).
  \end{align*}
  }
The consistency of this estimator follows from the consistency of
$\widehat{S}(a,b)$ for $S(a,b)$, Slutzky's theorem and the
continuous mapping theorem.
% \footnote{
% Alternatively, we could treat the terms in~\eqref{eqn:tsalliscdAsympVar}
% directly in the framework outlined in Section~\ref{sec:multipleDistros}. The
% resulting estimators require numerical integration which is not computationally
% desirable.}.

 

